Label Anchored Contrastive Learning for Language Understanding

Contrastive learning (CL) has achieved astonishing progress in computer vision, speech, and natural language processing fields recently with self-supervised learning. However, CL approach to the supervised setting is not fully explored, especially for the natural language understanding classification task. Intuitively, the class label itself has the intrinsic ability to perform hard positive/negative mining, which is crucial for CL. Motivated by this, we propose a novel label anchored contrastive learning approach (denoted as LaCon) for language understanding. Specifically, three contrastive objectives are devised, including a multi-head instance-centered contrastive loss (ICL), a label-centered contrastive loss (LCL), and a label embedding regularizer (LER). Our approach does not require any specialized network architecture or any extra data augmentation, thus it can be easily plugged into existing powerful pre-trained language models. Compared to the state-of-the-art baselines, LaCon obtains up to 4.1% improvement on the popular datasets of GLUE and CLUE benchmarks. Besides, LaCon also demonstrates significant advantages under the few-shot and data imbalance settings, which obtains up to 9.4% improvement on the FewGLUE and FewCLUE benchmarking tasks.

==> tabels.tex <==

\begin{table}[htp]
\centering
\small
\begin{tabular}{ccccc}
\hline \textbf{Methods} & \textbf{YelpBin} & \textbf{IMDB} & \textbf{SST-2} & \textbf{Weibo} \\ \hline
BERT & {82.05} & {86.9} & {91.22} & {97.4} \cr
LBS & {81.8} & {87.0} & {91.22} & {97.5} \cr
LEAM & {82.09} & {87.4} & {91.24} & {97.4} \cr
BAN & {82.14} & {86.9} & {91.18} & {97.4} \cr
R-DROP & \textbf{82.3} & {87.4} & \textbf{91.4} & \textbf{97.7} \cr
SCL & {81.4} & \textbf{87.8} & \textbf{91.4} & {97.5} \cr
\hline
LAFM & \textbf{82.3} & {87.2} & {91.06} & \textbf{97.7} \cr
\hline
\end{tabular}
\caption{The experimental results for sentiment analysis.}
\label{tab:exp-senti}
\end{table}

\begin{table}[htp]
\centering
\small
\begin{tabular}{cccc}
\hline \textbf{Methods} & \textbf{DBPedia} & \textbf{Agnews} & \textbf{Tnews}  \\ \hline
BERT & {96.15/92.63} & {83.53/83.39} & {54.33/51.67}  \cr
LBS & {96.37/92.01} & {83.72/83.45} & {54.4/52.74}  \cr
LEAM & {96.15/92.9} & {83.86/83.56} & {54.63/54.72}  \cr
BAN & {96.18/92.85} & {83.49/83.45} & {54.39/52.42}  \cr
R-DROP & {95.47/94.02} & {83.55/83.47} & {54.9/52.72}  \cr
SCL & {96.22/93.53} & {83.82/83.78} & {55.25/53.81} \cr
\hline
LAFM & \textbf{96.23/95.02} & \textbf{84.4/84.0} & \textbf{55.6/55.4} \cr
\hline
\end{tabular}
\caption{The experimental results for genre classification.}
\label{tab:exp-genre}
\end{table}

\begin{table}[htp]
\centering
\small
\begin{tabular}{ccccc}
\hline \textbf{Methods} & \textbf{MNLI} & \textbf{QNLI} & \textbf{RTE} & \textbf{OCNLI} \\ \hline
BERT & {72.54} & {87.16} & {67.32} & {67.39} \cr
LBS & {72.82} & {87.4} & {67.24} & {67.68} \cr
LEAM & {72.46} & {87.2} & {67.3} & {67.25} \cr
BAN & {72.39} & {87.0} & {67.18} & {67.92} \cr
R-DROP & {73.11} & {87.59} & {69.22} & \textbf{68.05} \cr
SCL & {72.86} & {87.73} & {69.13} & {67.49} \cr
\hline
LAFM & \textbf{73.25} & \textbf{88.06} & \textbf{71.38} & {67.69} \cr
\hline
\end{tabular}
\caption{The experimental results for NLI.}
\label{tab:exp-nli}
\end{table}

\begin{table}[htp]
\centering
\small
\begin{tabular}{ccccc}
\hline \textbf{Methods} & \textbf{QQP} & \textbf{MRPC} & \textbf{AFQMC} & \textbf{CoLA} \\ \hline
BERT & {82.25} & {85.63} & {72.76} & {60.91} \cr
LBS & {82.27} & {85.56} & {72.93} & {61.68} \cr
LEAM & {81.88} & {85.66} & {72.81} & {60.87} \cr
BAN & {82.39} & {85.62} & {72.63} & {60.83} \cr
R-DROP & {81.17} & {86.61} & {73.06} & {61.29} \cr
SCL & {82.48} & \textbf{88.08} & \textbf{74.16} & {62.26} \cr
\hline
LAFM & \textbf{82.8} & {87.16} & {73.2} & \textbf{62.36} \cr
\hline
\end{tabular}
\caption{The experimental results for PI and LA.}
\label{tab:exp-pi}
\end{table}



\begin{table*}[htp]
\centering
\small
\begin{tabular}{c|cccccccc}
\hline \textbf{Methods} & \textbf{YelpBin} & \textbf{IMDB} & \textbf{SST-2} & \textbf{Weibo} & \textbf{DBPedia} & \textbf{Agnews} & \textbf{Tnews} & \\ \hline
BERT & {82.05$\pm 0.45$} & {86.9$\pm 0.49$} & {91.22$\pm 0.06$} & {97.4$\pm 0.2$} & {92.63$\pm 1.18$} & {83.39$\pm 0.38$} & {51.67$\pm 0.08$}  \cr
LBS & {81.8$\pm 0.39 $} & {87.0$\pm 0.26$} & {91.22$\pm 0.46 $} & {97.5$\pm 0.12 $} & {92.01$\pm 0.15 $} & {83.45$\pm 0.2 $} & {52.74$\pm 0.79 $}  \cr
LEAM & {82.09$\pm 0.57 $} & {87.4$\pm 0.53 $} & {91.24$\pm 1.03 $} & {97.4$\pm 0.17 $}  & {92.9$\pm 0.77 $} & {83.56$\pm 0.45 $} & {54.72$\pm 0.52 $}  \cr
BAN & {82.14$\pm 1.52 $} & {86.9$\pm 0.93 $} & {91.18$\pm 0.74 $} & {97.4$\pm 1.10 $} & {92.85$\pm 0.92 $} & {83.45$\pm 0.21 $} & {52.42$\pm 0.53 $}  \cr
LSAN & { 82.21 $\pm 0.57 $} & { 87.05 $\pm  0.92 $} & { 91.03 $\pm 1.22 $} & { 97.4 $\pm 0.73 $} & { 93.75 $\pm 1.14 $} & { 83.91 $\pm 0.19 $} & { 54.99 $\pm 0.56  $}  \cr
R-DROP & \textbf{82.3$\pm 0.29 $} & {87.4$\pm 0.29 $} & \textbf{91.4$\pm 0.27 $} & \textbf{97.7$\pm 0.09 $} & {94.02$\pm 1.82 $} & {83.47$\pm 0.39 $} & {52.72$\pm 0.82 $}  \cr
SCL & {81.4$\pm 0.83 $} & \textbf{87.8$\pm 0.54 $} & \textbf{91.4$\pm 0.3 $} & {97.5$\pm 0.19 $} & {93.53$\pm 0.15 $} & {83.78$\pm 0.18 $} & {53.81$\pm 0.69 $} \cr
\hline
LAFM & \textbf{82.3$\pm 0.5 $} & {87.2$\pm 0.12 $} & {91.06$\pm 0.28 $} & \textbf{97.7$\pm 0.05 $} & \textbf{95.02$\pm 0.8 $} & \textbf{84.0$\pm 0.36 $} & \textbf{55.4$\pm 0.27 $} \cr
\hline
\\
\textbf{} & \textbf{MNLI} & \textbf{QNLI} & \textbf{RTE} & \textbf{OCNLI} & \textbf{QQP} & \textbf{MRPC} & \textbf{AFQMC} & \textbf{CoLA} \\ \hline

BERT & {72.54$\pm 0.3 $} & {87.16$\pm 0.22 $} & {67.32$\pm 1.92 $} & {67.39$\pm 0.29 $} & {82.25$\pm 0.48 $} & {85.63$\pm 1.56 $} & {72.76$\pm 0.25 $} & {60.91$\pm 0.78 $} \cr
LBS & {72.82$\pm 0.34 $} & {87.4$\pm 0.14 $} & {67.24$\pm 0.32 $} & {67.68$\pm 0.79 $}
& {82.27$\pm 0.12 $} & {85.56$\pm 1.21 $} & {72.93$\pm 0.11 $} & {61.68$\pm 0.72 $} \cr
LEAM & {72.46$\pm 0.51 $} & {87.2$\pm 0.68 $} & {67.3$\pm 1.29 $} & {67.25$\pm 0.61 $} 
& {81.88$\pm 0.45 $} & {85.66$\pm 1.33 $} & {72.81$\pm 0.24 $} & {60.87$\pm 1.01 $} \cr
BAN & {72.39$\pm 0.67 $} & {87.0$\pm 0.45 $} & {67.18$\pm 0.67 $} & {67.92$\pm 0.89 $} 
& {82.39$\pm 0.58 $} & {85.62$\pm 0.94 $} & {72.63$\pm 0.31 $} & {60.83$\pm 0.95 $} \cr
LSAN & { 72.93 $\pm 0.44 $} & { 87.05 $\pm 0.27 $} & { 69.76 $\pm 1.04 $} & { 67.86 $\pm 0.76 $} & { 81.15 $\pm 0.49 $} & { 86.05 $\pm 0.73 $} & { 72.46 $\pm 0.59  $} & { 61.67 $\pm 0.87  $}  \cr
R-DROP & {73.11$\pm 0.3 $} & {87.59$\pm 0.26 $} & {69.22$\pm 1.37 $} & \textbf{68.05$\pm 0.39 $}
& {81.17$\pm 0.17 $} & {86.61$\pm 1.03 $} & {73.06$\pm 2.01 $} & {61.29$\pm 0.63 $} \cr
SCL & {72.86$\pm 1.53 $} & {87.73$\pm 0.14 $} & {69.13$\pm 2.23 $} & {67.49$\pm 0.26 $}
& {82.48$\pm 0.62 $} & \textbf{88.08$\pm 0.86 $} & \textbf{74.16$\pm 1.1 $} & {62.26$\pm 0.59 $} \cr
\hline
LAFM & \textbf{73.25$\pm 0.36 $} & \textbf{88.06$\pm 0.16 $} & \textbf{71.38$\pm 0.73 $} & {67.69$\pm 0.66 $} 
& \textbf{82.8$\pm 0.0.52 $} & {87.47$\pm 0.88 $} & {73.2$\pm 0.3 $} & \textbf{62.36$\pm 1.08 $} \cr

\hline
\end{tabular}
\caption{The experimental results for Five Text classification Tasks. Best scores for each dataset are highlight in \textbf{bold}.}
\label{tab:exp-all}
\end{table*}



\begin{table*}[htp]
\centering
\small
\begin{tabular}{c|ccccccccc}
\hline \textbf{Methods} & \textbf{YelpRev} & \textbf{WOS}  & \textbf{DBPedia}  & \textbf{Tnews} &  \textbf{QNLI} & \textbf{RTE} & \textbf{QQP} & \textbf{MRPC} & \textbf{CoLA}  \\ \hline

CE   & {82.0$\pm 0.5$} & {85.0$\pm0.4$} & { 98.7$\pm0.3$ } & {54.5$\pm 0.3$}  & {87.1$\pm 0.2 $} & {67.3$\pm 1.9 $} &  {82.2$\pm 0.5 $} & {85.6$\pm 1.6 $} & {60.9$\pm 0.8 $} \cr

LEAM  & {82.1$\pm 0.6 $} & {85.1$\pm0.1$} & {98.7$\pm0.5$} & {54.1$\pm 0.3 $}  & {87.2$\pm 0.7 $} & {67.3$\pm 1.3 $} & {81.9$\pm 0.5 $} & {85.6$\pm 1.3 $} &  {60.9$\pm 1.0 $} \cr

LSAN  & { 82.2$\pm 0.6 $} & {85.2$\pm0.5$} & {98.7$\pm0.7$} & { 54.9$\pm 0.8  $} & { 87.1$\pm 0.3 $} & { 69.7$\pm 1.0 $} & { 81.2$\pm 0.5 $} & { 86.1$\pm 0.7 $} & { 61.6$\pm 0.9  $} \cr

CE+CL & {82.2$\pm0.6$} & {85.1$\pm0.4$} & {98.5$\pm0.5$} & {53.9$\pm0.5$} & {87.3$\pm0.3$} & {67.8$\pm1.5$} & {82.4$\pm0.3$} & {83.1$\pm0.7$} & {61.1$\pm0.7$} \cr

CE+SCL  & {81.4$\pm 0.8 $} & {84.8$\pm0.2$} & {98.5$\pm0.6$} & {54.6$\pm 0.2 $}  &  {87.7$\pm 0.1 $} & {69.1$\pm 2.2 $}
& {82.5$\pm 0.6 $} & \textbf{88.1$\pm 0.9 $} & {62.3$\pm 0.6 $} \cr

\hline
LaCon (vanilla)  &  \textbf{82.3$\pm 0.5 $}  & {} & \textbf{98.9$\pm0.5$} & \textbf{56.8$\pm 0.6 $}  & \textbf{88.1$\pm 0.2 $} & \textbf{71.4$\pm 0.7 $} & \textbf{82.8$\pm 0.5 $} & {87.5$\pm 0.9 $} & \textbf{62.4$\pm 1.0 $} \cr

LaCon w/ fusion &  \textbf{83.1$\pm 0.8 $}  & \textbf{$\pm 0.$} & \textbf{99.5$\pm0.2$} & \textbf{56.7$\pm 0.3$}  & \textbf{88.4$\pm 0.3$} & \textbf{72.2$\pm 0.9$} & \textbf{83.7$\pm 0.5$} & \textbf{88.6$\pm 0.7$} & \textbf{62.8$\pm0.5$} \cr

\hline
\end{tabular}
\caption{The experimental results for the Language Understanding Tasks. Best scores with significant value $p < 0.05$ for each dataset are highlight in \textbf{bold}.}

\label{tab:exp-all}
\end{table*}
